Semi-Supervised Model-Free Bayesian State Estimation from Compressed Measurements

We consider data-driven Bayesian state estimation from compressed measurements (BSCM) of a model-free process. The dimension of the temporal measurement vector is lower than that of the temporal state vector to be estimated, leading to an under-determined inverse problem. The underlying dynamical model of the state's evolution is unknown for a `model-free process.' Hence, it is difficult to use traditional model-driven methods, for example, Kalman and particle filters. Instead, we consider data-driven methods. We experimentally show that two existing unsupervised learning-based data-driven methods fail to address the BSCM problem in a model-free process. The methods are -- data-driven nonlinear state estimation (DANSE) and deep Markov model (DMM). While DANSE provides good predictive/forecasting performance to model the temporal measurement data as a time series, its unsupervised learning lacks suitable regularization for tackling the BSCM task. We then propose a semi-supervised learning approach and develop a semi-supervised learning-based DANSE method, referred to as SemiDANSE. In SemiDANSE, we use a large amount of unlabelled data along with a limited amount of labelled data, i.e., pairwise measurement-and-state data, which provides the desired regularization. Using {benchmark chaotic dynamical systems}, we {empirically} show that the data-driven SemiDANSE provides competitive state estimation performance for BSCM {using a handful of different measurement systems}, against a hybrid method called KalmanNet and two model-driven methods (extended Kalman filter and unscented Kalman filter) that know the dynamical models exactly.

==> figs/revision_1/LorenzSSMn2_nmse_vs_smnr_diff_train_SMNR.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkturquoise0191191}{RGB}{0,191,191}
\definecolor{goldenrod1911910}{RGB}{191,191,0}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.32,0.5)}, draw=lightgray204},
tick align=outside,
tick pos=left,
%title={\(\displaystyle {\sigma}_{e,{train}}^2 = -10.0\) dB},
x grid style={darkgray176},
xlabel={\textcolor{blue}{\(\displaystyle \text{SMNR}\) (in dB)}},
xmajorgrids,
xmin=-12, xmax=32,
xtick style={color=black},
xtick={-10,0,10,20,30},
xticklabels={
  %\(\displaystyle {\ensuremath{-}15}\),
  \(\displaystyle {\ensuremath{-}10}\),
  %\(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\),
  %\(\displaystyle {5}\),
  \(\displaystyle {10}\),
  %\(\displaystyle {15}\),
  \(\displaystyle {20}\),
  %\(\displaystyle {25}\),
  \(\displaystyle {30}\),
  %\(\displaystyle {35}\)
},
y grid style={darkgray176},
ylabel={\textcolor{blue}{NMSE (in dB)}},
ymajorgrids,
ymin=-31.8039075557143, ymax=0.310363163426518,
ytick style={color=black},
ytick={-35,-30,-25,-20,-15,-10,-5,0,5},
yticklabels={
  \(\displaystyle {\ensuremath{-}35}\),
  \(\displaystyle {\ensuremath{-}30}\),
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {\ensuremath{-}15}\),
  \(\displaystyle {\ensuremath{-}10}\),
  \(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\),
  \(\displaystyle {5}\)
},
width=0.49\textwidth,
height=0.4\textwidth
]
\path [draw=blue, semithick]
(axis cs:-10,-5.88740210235119)
--(axis cs:-10,-5.61858697235584);

\path [draw=blue, semithick]
(axis cs:0,-6.38814243674278)
--(axis cs:0,-5.87124553322792);

\path [draw=blue, semithick]
(axis cs:10,-8.97416996955872)
--(axis cs:10,-6.51535487174988);

\path [draw=blue, semithick]
(axis cs:20,-10.6246709823608)
--(axis cs:20,-8.62411212921143);

\path [draw=blue, semithick]
(axis cs:30,-10.8772591203451)
--(axis cs:30,-10.6820060163736);

\path [draw=red, semithick]
(axis cs:-10,-4.08694431185722)
--(axis cs:-10,-3.48816707730293);

\path [draw=red, semithick]
(axis cs:0,-8.35048897564411)
--(axis cs:0,-8.03161399066448);

\path [draw=red, semithick]
(axis cs:10,-9.91824667155743)
--(axis cs:10,-9.56631715595722);

\path [draw=red, semithick]
(axis cs:20,-12.5045158565044)
--(axis cs:20,-11.9647262394428);

\path [draw=red, semithick]
(axis cs:30,-12.9590139091015)
--(axis cs:30,-12.6983042061329);

\path [draw=green01270, semithick]
(axis cs:-10,-1.88767687231302)
--(axis cs:-10,-1.67547162622213);

\path [draw=green01270, semithick]
(axis cs:0,-8.21982881426811)
--(axis cs:0,-7.67175367474556);

\path [draw=green01270, semithick]
(axis cs:10,-16.2788741886616)
--(axis cs:10,-15.7997009456158);

\path [draw=green01270, semithick]
(axis cs:20,-17.7772634923458)
--(axis cs:20,-17.3913232386112);

\path [draw=green01270, semithick]
(axis cs:30,-18.5412397384644)
--(axis cs:30,-18.1070718765259);

\path [draw=goldenrod1911910, semithick]
(axis cs:-10,-2.62830413877964)
--(axis cs:-10,-2.38975082337856);

\path [draw=goldenrod1911910, semithick]
(axis cs:0,-8.31222657859325)
--(axis cs:0,-7.89544172585011);

\path [draw=goldenrod1911910, semithick]
(axis cs:10,-18.1221289634705)
--(axis cs:10,-17.638231754303);

\path [draw=goldenrod1911910, semithick]
(axis cs:20,-23.7322910279036)
--(axis cs:20,-23.248803332448);

\path [draw=goldenrod1911910, semithick]
(axis cs:30,-25.4439668059349)
--(axis cs:30,-24.7513228058815);

\path [draw=darkturquoise0191191, semithick]
(axis cs:-10,-1.34662196785212)
--(axis cs:-10,-1.14937641471624);

\path [draw=darkturquoise0191191, semithick]
(axis cs:0,-5.84085047245026)
--(axis cs:0,-5.47700536251068);

\path [draw=darkturquoise0191191, semithick]
(axis cs:10,-16.225137501955)
--(axis cs:10,-15.847128123045);

\path [draw=darkturquoise0191191, semithick]
(axis cs:20,-25.4413353800774)
--(axis cs:20,-25.1431944966316);

\path [draw=darkturquoise0191191, semithick]
(axis cs:30,-30.3441679775715)
--(axis cs:30,-29.8260667026043);

\path [draw=black, semithick]
(axis cs:-10,-5.88740263879299)
--(axis cs:-10,-5.6186131387949);

\path [draw=black, semithick]
(axis cs:0,-8.3504486232996)
--(axis cs:0,-8.03160475194454);

\path [draw=black, semithick]
(axis cs:10,-16.2809309214354)
--(axis cs:10,-15.8039766103029);

\path [draw=black, semithick]
(axis cs:20,-23.7295204550028)
--(axis cs:20,-23.2397483438253);

\path [draw=black, semithick]
(axis cs:30,-30.3293041586876)
--(axis cs:30,-29.8112483620644);
\addplot [semithick, line width=1, black, mark=square, mark size=3, mark options={solid,fill opacity=0}]
table {%
-10 -5.75300788879395
0 -8.19102668762207
10 -16.0424537658691
20 -23.4846343994141
30 -30.070276260376
};
\addlegendentry{\textcolor{blue}{Matched}}
\addplot [semithick, line width=1, blue, dashdotted, mark=triangle, mark size=3, mark options={solid,rotate=180,fill opacity=0}]
table {%
-10 -5.75299453735352
0 -6.12969398498535
10 -7.7447624206543
20 -9.62439155578613
30 -10.7796325683594
};
\addlegendentry{\textcolor{blue}{$-10 $ dB}}
\addplot [semithick, line width=1, red, dashdotted, mark=o, mark size=3, mark options={solid,fill opacity=0}]
table {%
-10 -3.78755569458008
0 -8.1910514831543
10 -9.74228191375732
20 -12.2346210479736
30 -12.8286590576172
};
\addlegendentry{\textcolor{blue}{$0 $ dB}}
\addplot [semithick, line width=1, green01270, dashdotted, mark=pentagon, mark size=3, mark options={solid,fill opacity=0}]
table {%
-10 -1.78157424926758
0 -7.94579124450684
10 -16.0392875671387
20 -17.5842933654785
30 -18.3241558074951
};
\addlegendentry{\textcolor{blue}{$10 $ dB}}
\addplot [semithick, line width=1, goldenrod1911910, dashdotted, mark=star, mark size=4, mark options={solid,fill opacity=0}]
table {%
-10 -2.5090274810791
0 -8.10383415222168
10 -17.8801803588867
20 -23.4905471801758
30 -25.0976448059082
};
\addlegendentry{\textcolor{blue}{$20 $ dB}}
\addplot [semithick, line width=1, darkturquoise0191191, dashdotted, mark=diamond, mark size=3, mark options={solid,fill opacity=0}]
table {%
-10 -1.24799919128418
0 -5.65892791748047
10 -16.0361328125
20 -25.2922649383545
30 -30.0851173400879
};
\addlegendentry{\textcolor{blue}{$30 $ dB}}
\end{axis}

\end{tikzpicture}


==> figs/revision_1/LorenzSSMrn2_nmse_vs_smnr_diff_kappa.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkturquoise0191191}{RGB}{0,191,191}
\definecolor{goldenrod1911910}{RGB}{191,191,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={SMNR (in dB)},
xmajorgrids,
xmin=-12, xmax=32,
xtick style={color=black},
xtick={-15,-10,-5,0,5,10,15,20,25,30,35},
xticklabels={
  \(\displaystyle {\ensuremath{-}15}\),
  \(\displaystyle {\ensuremath{-}10}\),
  \(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\),
  \(\displaystyle {5}\),
  \(\displaystyle {10}\),
  \(\displaystyle {15}\),
  \(\displaystyle {20}\),
  \(\displaystyle {25}\),
  \(\displaystyle {30}\),
  \(\displaystyle {35}\)
},
y grid style={darkgray176},
ylabel={NMSE (in dB)},
ymajorgrids,
ymin=-30.6581974066794, ymax=-3.003094535321,
ytick style={color=black},
ytick={-35,-30,-25,-20,-15,-10,-5,0},
yticklabels={
  \(\displaystyle {\ensuremath{-}35}\),
  \(\displaystyle {\ensuremath{-}30}\),
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {\ensuremath{-}15}\),
  \(\displaystyle {\ensuremath{-}10}\),
  \(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\)
},
width=0.49\textwidth,
height=0.45\textwidth
]
\path [draw=blue, semithick]
(axis cs:-10,-4.60302595794201)
--(axis cs:-10,-4.26014466583729);

\path [draw=blue, semithick]
(axis cs:0,-6.95517072081566)
--(axis cs:0,-6.48572054505348);

\path [draw=blue, semithick]
(axis cs:10,-14.8834634423256)
--(axis cs:10,-13.8989691138268);

\path [draw=blue, semithick]
(axis cs:20,-21.5537815690041)
--(axis cs:20,-20.8015498518944);

\path [draw=blue, semithick]
(axis cs:30,-25.9403686523438)
--(axis cs:30,-23.7058715820312);

\path [draw=goldenrod1911910, semithick]
(axis cs:-10,-5.69197844713926)
--(axis cs:-10,-5.45718003064394);

\path [draw=goldenrod1911910, semithick]
(axis cs:0,-6.62669973820448)
--(axis cs:0,-6.45555276423693);

\path [draw=goldenrod1911910, semithick]
(axis cs:10,-14.0617950558662)
--(axis cs:10,-13.2911903262138);

\path [draw=goldenrod1911910, semithick]
(axis cs:20,-22.7357324063778)
--(axis cs:20,-21.7943235933781);

\path [draw=goldenrod1911910, semithick]
(axis cs:30,-29.0610977709293)
--(axis cs:30,-28.2616866528988);

\path [draw=darkturquoise0191191, semithick]
(axis cs:-10,-5.7485224455595)
--(axis cs:-10,-5.5112431794405);

\path [draw=darkturquoise0191191, semithick]
(axis cs:0,-6.75100007653236)
--(axis cs:0,-6.57665953040123);

\path [draw=darkturquoise0191191, semithick]
(axis cs:10,-15.6647585630417)
--(axis cs:10,-12.1750127077103);

\path [draw=darkturquoise0191191, semithick]
(axis cs:20,-22.1473042368889)
--(axis cs:20,-21.0357096791267);

\path [draw=darkturquoise0191191, semithick]
(axis cs:30,-29.4011472761631)
--(axis cs:30,-28.8737321794033);

\addplot [semithick, blue, mark=triangle, mark size=6, mark options={solid,rotate=180,fill opacity=0}]
table {%
-10 -4.43158531188965
0 -6.72044563293457
10 -14.3912162780762
20 -21.1776657104492
30 -24.8231201171875
};
\addlegendentry{Semi-DANSE $ (\kappa=5\%)$}
\addplot [semithick, goldenrod1911910, mark=square, mark size=6, mark options={solid,fill opacity=0}]
table {%
-10 -5.5745792388916
0 -6.5411262512207
10 -13.67649269104
20 -22.2650279998779
30 -28.6613922119141
};
\addlegendentry{Semi-DANSE $ (\kappa=5\%)$}
\addplot [semithick, darkturquoise0191191, mark=pentagon, mark size=6, mark options={solid,fill opacity=0}]
table {%
-10 -5.6298828125
0 -6.6638298034668
10 -13.919885635376
20 -21.5915069580078
30 -29.1374397277832
};
\addlegendentry{Semi-DANSE $ (\kappa=5\%)$}
\end{axis}

\end{tikzpicture}


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
